Bidirectional Type Slicing

Development tools report what type an expression has, but not why it has that type. This paper develops a theory of type slicing: a programmer selects a term, queries any part of its type information, and receives a program slice that is sufficient to reproduce the queried type. We formulate type slicing for bidirectional type systems, where synthesis slices explain the type a term synthesises and analysis slices explain the type expected by its surrounding context. The theory applies to any bidirectional system equipped with precision orders on types and terms satisfying a downwards static graduality property. We develop the metatheory over a core calculus with holes, products, sums, and explicit polymorphism, based on the Hazelnut and marked lambda calculi. We prove that every query has a minimal slice and that refining a query monotonically shrinks its minimal slices. We then show how to calculate these slices both exactly and approximately. Finally, integrating type slicing with error marking theory extends these results to arbitrary ill-typed programs, so a single mechanism explains both types and type errors in complete, incomplete, and erroneous code. The metatheory is mechanised in Agda, and a linear-time approximation of type slicing is implemented for the Hazel programming environment.

==> preamble.tex <==











\let\Bbbk\relax
\usepackage{amssymb}


\let\sqsubseteqOriginal\sqsubseteq
\let\sqsupseteqOriginal\sqsupseteq

\usepackage{semantic}        








\makeatletter
\newdimen\sem@defaultrulethick
\sem@defaultrulethick=0.4pt
\patchcmd{\@inferenceBack}
  {\vskip 4\fontdimen8\textfont3}{\vskip 4\sem@defaultrulethick}
  {}{\PackageWarning{preamble}{semantic \string\inference\space patch 1 failed}}
\patchcmd{\@inferenceBack}
  {\vskip 4\fontdimen8\textfont3}{\vskip 4\sem@defaultrulethick}
  {}{\PackageWarning{preamble}{semantic \string\inference\space patch 2 failed}}
\patchcmd{\@processInference}
  {\advance\dimen3 by \fontdimen8\textfont3}
  {\advance\dimen3 by \sem@defaultrulethick}
  {}{\PackageWarning{preamble}{semantic \string\inference\space patch 3 failed}}
\makeatother

\usepackage{stmaryrd}        
\providecommand{\Circle}{\bigcirc} 
\usepackage{mathtools}


\makeatletter
\newcommand{\priorDissertationSelfCite}{
  \if@ACM@anonymous
    \cite{AnonymousDissertation2025}
  \else
    \cite{Carroll2025}
  \fi}
\newcommand{\hatraSelfCite}{
  \if@ACM@anonymous
    \cite{AnonymousHATRA2025}
  \else
    \cite{CarrollEtAl2025}
  \fi}
\makeatother




\makeatletter
\@ifpackageloaded{unicode-math}{
  \setmathfont{latinmodern-math.otf}[range={"023DE,"023DF},Scale=MatchLowercase]
}{}
\makeatother

\usepackage{soul}             
\usepackage[most]{tcolorbox}
\usepackage[normalem]{ulem}

\usepackage{tabularx}
\usepackage{arydshln}         
\usepackage{float}
\usepackage{subcaption}

\usepackage{etoolbox}
\usepackage{needspace}






\usepackage[capitalise]{cleveref}


\crefname{section}{Sec.}{Secs.}
\Crefname{section}{Section}{Sections}




\definecolor{commentgreen}{RGB}{2,112,10}
\definecolor{weborange}{RGB}{255,165,0}
\definecolor{frenchplum}{RGB}{129,20,83}


\definecolor{BrickRed}{RGB}{210,35,40}
\definecolor{NavyBlue}{RGB}{30,80,225}
\definecolor{OliveGreen}{RGB}{35,165,45}
\definecolor{Mulberry}{RGB}{215,55,175}


\colorlet{assumed}{BurntOrange!80!black}
\colorlet{induced}{TealBlue!45!black}







\newcommand{\edited}[1]{#1}
\newtcolorbox{editedblock}{breakable, enhanced, colback=cyan!6, colframe=cyan!45,
  boxrule=0.3pt, left=4pt, right=4pt, top=3pt, bottom=3pt, sharp corners}




\newcommand{\asmref}[1]{\textcolor{assumed}{\textbf{#1}}}
\newcommand{\synsrc}[1]{\textcolor{NavyBlue!60!gray}{#1}}
\newcommand{\anasrc}[1]{\textcolor{OliveGreen!60!gray}{#1}}



\newcommand{\heavymono}{\bfseries\ttfamily}
\newcommand{\synsrcS}[1]{\textcolor{blue!85!black}{{\heavymono #1}}}
\newcommand{\anasrcS}[1]{\textcolor{OliveGreen!75!black}{{\heavymono #1}}}
\newcommand{\strN}[1]{\textcolor{black!85}{#1}}


\newcommand{\fold}{\gap}




\definecolor{latticecolor}{HTML}{8055B5}
\let\OLDsqcap\sqcap
\let\OLDsqcup\sqcup
\let\OLDsqsubset\sqsubset
\let\OLDsqsupset\sqsupset
\def\sqcap{\mathbin{{\color{latticecolor}\OLDsqcap}}}
\def\sqcup{\mathbin{{\color{latticecolor}\OLDsqcup}}}
\def\sqsubseteq{\mathrel{{\color{latticecolor}\sqsubseteqOriginal}}}
\def\sqsupseteq{\mathrel{{\color{latticecolor}\sqsupseteqOriginal}}}
\def\sqsubset{\mathrel{{\color{latticecolor}\OLDsqsubset}}}
\def\sqsupset{\mathrel{{\color{latticecolor}\OLDsqsupset}}}
\newcommand{\heytingto}{\ensuremath{\mathbin{{\color{latticecolor}\to}}}}
\newcommand{\heytingminus}{\ensuremath{\mathbin{{\color{latticecolor}\setminus}}}}
\newcommand{\latticetop}{\ensuremath{{\color{latticecolor}\top}}}
\newcommand{\latticebot}{\ensuremath{{\color{latticecolor}\bot}}}




\newcommand{\hlc}[2][yellow]{{
    \colorlet{foo}{#1}
    \sethlcolor{foo}\hl{#2}}
}
\newcommand{\error}[1]{\hlc[pink!50]{#1}}
\newcommand{\hlcmaths}[2][yellow!50]{\colorbox{#1}{$\displaystyle #2$}}

\newcommand{\dyn}{{\color{teal}\texttt{?}}}          
\newcommand{\gap}{\ensuremath{{\color{teal}\Box}}}
\newcommand{\hole}[1][]{\ensuremath{{\color{teal}\llparenthesis} #1 {\color{teal}\rrparenthesis}}} 
\newcommand{\cmark}{\ensuremath{{\color{blue}\Circle}}}            
\newcommand{\type}[1]{\llbracket #1 \rrbracket}       
\newcommand{\id}{\mathrm{id}}
\newcommand{\code}[1]{\texttt{#1}}


\newcommand{\wf}[2][\Delta]{#1 \vdash #2\;\mathsf{wf}}


\newcommand{\funarr}{\ensuremath{\mathbin{\to}}}
\newcommand{\synmode}{\ensuremath{\mathrel{{\color{BrickRed}\Rightarrow}}}}
\newcommand{\anamode}{\ensuremath{\mathrel{{\color{BlueViolet}\Leftarrow}}}}
\newcommand{\synthesis}[3][\Delta;\,\Gamma]{#1 \vdash #2 \synmode #3}
\newcommand{\analysis}[3][\Delta;\,\Gamma]{#1 \vdash #2 \anamode #3}


\newcommand{\synr}[1]{\textnormal{$\synmode$\texttt{#1}}}
\newcommand{\anar}[1]{\textnormal{$\anamode$\texttt{#1}}}
\newcommand{\cnsr}[1]{\textnormal{$#1$}}

\newcommand{\typeassignment}[3][\Delta;\Gamma]{#1 \vdash #2 : #3}


\newcommand{\synthesisslice}[4][\Gamma]{#1 \vdash #2 \synmode #3 \mid #4}
\newcommand{\analysisslice}[5][\Gamma]{#1; #2 \vdash #3 \anamode #4 \mid #5}


\providecommand{\tmrule}[7][\Delta;\,\Gamma]{
  #1 \vdash #2 \mathbin{\synmode} #3
  \mathbin{{\color{BrickRed}\blacktriangleleft}} #4
  \;{\color{BrickRed}\rightsquigarrow}\; #5
  \mathbin{\synmode} #6
  \,\dashv\, #7
}


\newcommand{\scast}[2]{{\color{blue}\langle} #1 {\color{blue}\Rightarrow} #2 {\color{blue}\rangle}}
\newcommand{\scasterror}[2]{{\color{red}\langle} #1 {\color{red}\Rightarrow} \dyn {\color{red}\nRightarrow} #2 {\color{red}\rangle}}
\newcommand{\scastcast}[3]{{\color{blue}\langle} #1 {\color{blue}\Rightarrow} #2 {\color{blue}\Rightarrow} #3 {\color{blue}\rangle}}


\newcommand{\funmatch}{\blacktriangleright_\rightarrow}
\newcommand{\groundmatch}{\blacktriangleright_{\text{ground}}}
\newcommand{\forallmatch}{\blacktriangleright_\forall}


\newcommand{\elaborationSynthesis}[5][\Gamma]{#1 \vdash #2 \synmode #3 \leadsto #4 \dashv #5}
\newcommand{\elaborationAnalysis}[6][\Gamma]{#1 \vdash #2 \anamode #3 \leadsto #4 : #5 \dashv #6}
\newcommand{\elaborationSynthesisSlice}[6][\Gamma]{#1 \vdash #2 \synmode #3 \mid #4 \leadsto #5 \dashv #6}
\newcommand{\elaborationAnalysisSlice}[9][\Gamma]{#1;\ #2 \vdash #3 \anamode #4 \mid #5 \leadsto #6 : #7 \mid #8 \dashv #9}


\newcommand{\ctxclass}[5][\Delta;\,\Gamma]{#1 \vdash #2\;\mathbf{at}\;#3\;\triangleright\;#4\;[\,#5\,]}


\newcommand{\marksto}{\looparrowright}
\newcommand{\synmark}[4][\Delta;\,\Gamma]{#1 \vdash #2 \marksto #3 \synmode #4}
\newcommand{\anamark}[4][\Delta;\,\Gamma]{#1 \vdash #2 \marksto #3 \anamode #4}
\newcommand{\mctxclass}[6][\Delta;\,\Gamma]{#1 \vdash #2 \marksto #3\;\mathbf{at}\;#4\;\triangleright\;#5\;[\,#6\,]}
\newcommand{\chk}[1]{\check{#1}}


\definecolor{markcolor}{RGB}{170,40,60}
\newcommand{\markopen}{{\color{markcolor}\llparenthesis}}
\newcommand{\markclose}{{\color{markcolor}\rrparenthesis}}
\newcommand{\markincon}[3][\cdot]{{\markopen #1 \markclose}_{#2 \not\sim #3}}
\newcommand{\markarrow}[1][\cdot]{{\markopen #1 \markclose}_{\blacktriangleright \funarr}}
\newcommand{\marksum}[1][\cdot]{{\markopen #1 \markclose}_{\blacktriangleright +}}
\newcommand{\markprod}[1][\cdot]{{\markopen #1 \markclose}_{\blacktriangleright \times}}
\newcommand{\markforall}[1][\cdot]{{\markopen #1 \markclose}_{\blacktriangleright \forall}}
\newcommand{\marklam}[1][\cdot]{{\markopen #1 \markclose}_{\sim \funarr}}
\newcommand{\markprodsim}[1][\cdot]{{\markopen #1 \markclose}_{\sim \times}}
\newcommand{\markvar}[1]{{\color{markcolor}\langle} #1 {\color{markcolor}\rangle}\!\synmode}

\newcommand{\markbox}[1]{
  \tikz[baseline=(N.base)]{
    \node[draw=BrickRed!85, line width=0.7pt, rounded corners=2pt,
          inner sep=2pt, fill=BrickRed!6, anchor=base] (N) {\strut$#1$};
  }
}

\DeclareRobustCommand{\squiggle}[1]{
  {\color{red}\uwave{\mbox{\normalcolor #1}}}
}

\newcommand{\slist}[1]{
  \tikz[baseline=(N.base)]{
    \node[draw=OliveGreen!25, dashed, line width=0.4pt, rounded corners=1.5pt,
          inner sep=1.5pt, fill=OliveGreen!4, anchor=base] (N) {\strut$#1$};
  }
}

\newcommand{\queryblock}[2]{
  \begin{center}
  \small
  \begin{tabular}{r@{\;}c@{\;}l}
    {\color{NavyBlue}synthesis query}  & $\upsilon\;=$ & $#1$ \\
    {\color{OliveGreen}analysis query} & $\psi\;=$ & $#2$ \\
  \end{tabular}
  \end{center}
}


\newcommand{\C}{\mathcal{C}}
\newcommand{\Cs}{c}
\newcommand{\p}{d}
\newcommand{\F}{\mathcal{F}}
\newcommand{\f}{f}
\newcommand{\Sb}{\mathcal{S}}

\DeclareMathAlphabet{\mathdcal}{U}{dutchcal}{m}{n}
\newcommand{\A}{\mathdcal{A}}

\newcommand{\ground}[1][\tau]{#1\text{ ground}}
\newcommand{\final}[1][d]{#1\text{ final}}
\newcommand{\val}[1][d]{#1\text{ val}}
\newcommand{\boxedval}[1][d]{#1\text{ boxedval}}
\newcommand{\indet}[1][d]{#1\text{ indet}}

\newcommand{\contextualsub}[1][d/u]{\llbracket #1 \rrbracket}


\newcommand{\Forall}[2]{\forall #1.\ #2}
\newcommand{\TLam}[2]{\Lambda #1.\ #2}
\newcommand{\TApp}[2]{#1\ @#2}
\newcommand{\ForallSlice}[2]{\forall #1.\ #2}
\newcommand{\gapforall}{{\color{teal}\forall\Box.\Box}}


\newcommand{\lbl}[2]{\mathtt{#1} : #2}
\newcommand{\tuplety}[1]{\{#1\}}





\makeatletter
\theoremstyle{acmplain}
\@ifundefined{theorem}{\newtheorem{theorem}{Theorem}[section]}{}
\@ifundefined{lemma}{\newtheorem{lemma}[theorem]{Lemma}}{}
\@ifundefined{proposition}{\newtheorem{proposition}[theorem]{Proposition}}{}
\@ifundefined{corollary}{\newtheorem{corollary}[theorem]{Corollary}}{}
\@ifundefined{conjecture}{\newtheorem{conjecture}[theorem]{Conjecture}}{}
\@ifundefined{counterexample}{\newtheorem{counterexample}[theorem]{Counterexample}}{}
\theoremstyle{acmdefinition}
\@ifundefined{definition}{\newtheorem{definition}[theorem]{Definition}}{}
\@ifundefined{example}{\newtheorem{example}[theorem]{Example}}{}
\theoremstyle{acmplain}
\@ifundefined{remark}{\newtheorem{remark}[theorem]{Remark}}{}
\makeatother


\newcounter{subthm}
\newcommand{\masterthmnum}{??}
\renewcommand{\thesubthm}{\masterthmnum.\arabic{subthm}}
\newcommand{\mastercases}{
  \xdef\masterthmnum{\thetheorem}
  \setcounter{subthm}{0}
}
\newenvironment{thmcase}[1][]{
  \refstepcounter{subthm}
  \par\medskip\noindent{\bfseries Theorem~\thesubthm}
  \ifx\\#1\\\else\ (\textit{#1})\fi
  {\bfseries.}\itshape\quad\ignorespaces
}{
  \par\medskip
}

\newtcolorbox{recipe}[1]{
  colback=blue!3, colframe=blue!40, fonttitle=\bfseries,
  title={Recipe: #1}, sharp corners, boxrule=0.5pt
}
\newtcolorbox{originalerror}[1][]{
  colback=red!3, colframe=red!40, fonttitle=\bfseries,
  title={Error (Original)#1}, sharp corners, boxrule=0.5pt
}
\newtcolorbox{majortheorembox}{
  colback=green!3, colframe=OliveGreen!60, sharp corners, boxrule=0.5pt, enhanced
}
\newtcolorbox{counterexamplebox}{
  colback=orange!3, colframe=orange!50, sharp corners, boxrule=0.5pt, enhanced
}


\newcommand{\sliceA}[1]{\textbf{\underline{\textcolor{BrickRed}{#1}}}}
\newcommand{\sliceB}[1]{\underline{\textcolor{NavyBlue}{#1}}}
\newcommand{\sliceC}[1]{\underline{\textcolor{OliveGreen}{#1}}}
\newcommand{\sliceD}[1]{\underline{\textcolor{Mulberry}{#1}}}




\makeatletter
\def\sli@olive{OliveGreen}
\def\sli@teal{teal}
\newcommand{\sli}[2][NavyBlue]{
  \def\sli@c{#1}
  \def\sli@style{dashed}
  \ifx\sli@c\sli@olive \def\sli@style{dotted}\fi
  \ifx\sli@c\sli@teal  \def\sli@style{densely dashdotted}\fi
  \tikz[baseline=(N.base)]{
    \node[draw=#1!60, \sli@style, line width=0.5pt, rounded corners=1.5pt,
          inner sep=1.5pt, fill=#1!12, anchor=base] (N) {\strut$#2$};
  }
}
\makeatother
\newcommand{\slr}[1]{
  \tikz[baseline=(N.base)]{
    \node[draw=BrickRed!80, line width=0.8pt, rounded corners=2pt,
          inner sep=3pt, fill=none, anchor=base] (N) {\strut$#1$};
  }
}
\newcommand{\fullslice}[2]{
  \begin{tikzpicture}[baseline=(t.base), every node/.style={inner sep=3pt}]
    \node[draw, line width=0.9pt, rounded corners,
          label={[font=\scriptsize\itshape]above:assumptions}] (a) {$#1$};
    \node[below=6pt of a] (t) {$#2$};
  \end{tikzpicture}
}
\newcommand{\gapbox}{\boxdot}


\usepackage{tikz-cd}
\usetikzlibrary{positioning,calc,fit,backgrounds,decorations.pathmorphing,shapes.geometric,arrows.meta}
\tikzcdset{arrows={->}, diagrams={column sep=large, row sep=large}}









\newcommand{\yo}{}
\newcommand{\no}{}
\newcommand{\po}{}
\newcommand{\iy}{}
\newcommand{\ino}{}
\newcommand{\ipart}{}
\newcommand{\mech}[2]{}
\newcommand{\mechyes}[1]{}
\newcommand{\mechno}[1]{}
\newcommand{\mechpartial}[1]{}
\newcommand{\mechfile}[2][]{}
\newcommand{\mechbox}[1]{}
\newcommand{\sectionlegend}{}

\makeatletter
\renewcommand{\marginpar}[2][]{}
\newcommand{\marginnote}[2][]{\@ifnextchar[\@mn@gobble\relax}
\def\@mn@gobble[#1]{}
\makeatother

